Continual learning of longitudinal health records

Continual learning denotes machine learning methods which can adapt to new environments while retaining and reusing knowledge gained from past experiences. Such methods address two issues encountered by models in non-stationary environments: ungeneralisability to new data, and the catastrophic forgetting of previous knowledge when retrained. This is a pervasive problem in clinical settings where patient data exhibits covariate shift not only between populations, but also continuously over time. However, while continual learning methods have seen nascent success in the imaging domain, they have been little applied to the multi-variate sequential data characteristic of critical care patient recordings. Here we evaluate a variety of continual learning methods on longitudinal ICU data in a series of representative healthcare scenarios. We find that while several methods mitigate short-term forgetting, domain shift remains a challenging problem over large series of tasks, with only replay based methods achieving stable long-term performance. Code for reproducing all experiments can be found at https://github.com/iacobo/continual

==> lit_review.tex <==
\paragraph{Formal definition} Formally we define a continual learning problem like so: Given a (possibly infinite) set of ordered tasks $T_i$ with associated datasets $(x_i, y_i)$ drawn from populations $(X_i, Y_i)$, and initial model $f_0$, for each $i$ we update $f_{i-1}$ on a subset of points from $(x_i,y_i)$ (the \textit{training set}) to obtain $f_{i-1} \rightarrow f_i$.

\begin{table}[ht]
\centering
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{l|lll}
         & Task Incremental & Class Incremental          & Domain Incremental      \\ \hline
Task 1   & $f(x) \in Y_1$ & $f(x) \in Y_1$                 & $f(x) \in Y, x \in X_1$ \\
Task 2   & $f(x) \in Y_2$ & $f(x) \in Y_2 \supset Y_1$     & $f(x) \in Y, x \in X_2$ \\
\multicolumn{1}{c|}{...}   &  \multicolumn{3}{c}{...}                        \\
Task $n$ & $f(x) \in Y_n$ & $f(x) \in Y_n \supset Y_{n-1}$ & $f(x) \in Y, x \in X_n$
\end{tabular}
\end{adjustbox}
\caption{A formalisation of the three Continual Learning scenarios in terms of model $f()$, input data $x$, population input data $X_i$, and target sets $Y_i$.}
\label{tab:formal-def-cl}
\end{table}


\begin{figure}[h]
	\centering
	\includegraphics[width=10cm]{figs/fig3}
	\caption{A high-level overview of the training and evaluation domains of related machine learning paradigms. In a traditional supervised learning context, we train and evaluate a model on one task with data drawn from a single distribution (grey). In \textit{transfer} learning we take an off-the-shelf model pre-trained on a related but distinct task (light blue) as a warm-start for training on our current task (grey). In \textit{multi-task} learning we train a model on multiple tasks simultaneously (dark blue, light blue, grey) but generally we are only interested in the model's performance on one of these (grey). These methods are all similar in that they exploit correlation in the learned features for multiple tasks to improve performance on a given task; the difference between these and \textit{continual} learning is the additional requirement that the model perform well on \textbf{all} previous tasks.}
	\label{fig:figs/train-val-test} 
\end{figure}








\subsection{Continual Learning in healthcare}
\label{sec:related-medical}

Healthcare has been frequently identified as a field prone to distribution shift from training data to deployment \citep{thiagarajan2018understanding, farquhar2018towards, lee2020clinical}. Domain adaptation has been extensively studied in this field, however such methods are also susceptible to Catastrophic Forgetting \citep{goodfellow2013empirical}, with the additional burden of requiring domain specific labels (which cannot always be guaranteed), and reliance on expert intervention during model specification.

Successful continual learning would allow the deployment of models which can incrementally adapt to broader ranges of patient data encountered, constantly generalising its 

Continual learning has thus far almost exclusively been applied to imaging medical data, with limited focus given to sequential data \cite{lenga2020continual}. However a large proportion of EHR exists in the form of tabular longitudinal data \citep{tayefi2021challenges}. In spite of this the authors are aware of only one prior study into CL as applied to such data \cite{kiyasseh2020continual}, a replay method applied to cardiac signals. Additionally, many scenarios in which they have been employed are artificial, with limited information on how well such methods scale to realistic problem statements.

Hurdles include limited standardisation of task definitions, availability of standardised datasets \citep{mimic21shengpu, harutyunyan2019multitask}, and a lack of method implementations compatible with sequential models. Further barriers to development include strict legislation governing the adaptation of algorithmic healthcare tools once deployed, a core concept in continually learning models \citep{vokinger2021continual}.

For a full review of CL methods as applied to medical data, see \citet{lee2020clinical}.

\subsection{Continual Learning in sequential data}
\label{sec:related-seq}

\paragraph{CL in sequential data} For a thorough evaluation of CL methods on sequential data generally, we refer to \citet{cossu2021continual}.

\subsection{Predictive task definitions in healthcare}
\label{sec:related-medical-ml}

While interest in machine learning applications to healthcare and clinical scenarios has sky-rocketed in recent years, standardisation of benchmarks, problem definitions, data processing remains low. Open access ICU datasets are limited, and works employing them vary wildly in experimental setups. To encourage reproducibility, we employ the FIDDLE \citep{mimic21shengpu} pre-processed ICU datasets derived from the commonly used MIMIC-III \citep{johnson2016mimic} and eICU-CRD \citep{eicu-crd-2.0}.

% Lit search "machine learning" AND (clinical OR healthcare OR ehr OR "electronic health records") AND (ICU)
% https://pubmed.ncbi.nlm.nih.gov/?term=%28machine+learning%29+AND+%28ICU%29
% Present table of:
% Predictive task | hours to prediction | Taken from first admission window | Num publications
% ICU datasets | Open access | Credentialed access | Year published | Data dims


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Clinical scenarios}
\label{sec:problem-def}

Clinical data undergoes covariate shift when source and target datasets are drawn from different populations, or from an evolving population over time. Here we consider three broad types of distribution: Models are typically developed using data from one or a small number of related institutions, but with the intention of deployment generally at an institution level. To simulate the setting of a model trained on datasets from multiple institutions throughout its training lifecycle, we propose the following 

To emulate a live evaluation scenario, ideally we would split the training and test data for each task temporally (see fig \ref{fig:figs/split-by-time}). However, due to anonymisation requirements of the MIMIC-3 and eICU-CRD datasets, patient admission dates are obfuscated, making such ordering of the data impossible.\footnote{This also prevents us exploring more robust temporal domain shifts (e.g. data split annually).}

% Standardisation of datasets / problem definition
% Meaningful task definitions
% There are a number of demographic splits seen in patient ICU data, however only a small subset of these meaningfully correspond to domain shifts encountered in the real world...

% Talk about how problems are usually defined (MENTION BENCHMARKS e.g. PMNIST, split mnist, CoRE50) in other CL settings, mention challenges of medical setting, type1 type2 error, metrics etc then segue into our definitions.

As per \cite{farquhar2018towards}, a number of existing benchmarks for continual learning methods do not adequately evaluate performance in real world scenarios e.g. ...

This is particularly pertinent to the medical domain, where 

%approval of devices undergoes strict assessment and where scope is rigidly defined. While offline \textit{multi-task} training has been shown to mutually improve automatic feature detection with even seemingly heterogeneous/disparate tasks, it is not clear how such a mechanism would be deployed in an online (\textit{continual learning}) clinical environment, where a given device is expected to perform a specific diagnostic, and information on distinct tasks is not routinely collected. (and tasks are encountered sequentially by the same device.)???

More readily apparent is the utility of \textit{domain incremental problems} where the task is nominally the same but there distribution shift is exhibited between training data and groups of online samples encountered through deployment (ref \ref{sec:domain-shift}).


To this end, we adapt a series of standard ICU predictive tasks derived from the open-access MIMIC-3 and eICU datasets to realistic Continual Learning problems. We define a Class Incremental problem, and three categories of Domain Incremental problem. All problems consist of a series of sequentially encountered tasks $T_i$, with associated datasets $D_i := \{X_i,Y_i\}$. For domain incremental problems, the set of $Y_i$ values is identical between tasks, but $X_i$ are drawn from different sub-populations. For Class incremental problems the target values additionally change. For a formalisation of this, see table \ref{tab:formal-def-cl}.

%For standardisatio  \textit{multi-task} EHR problem-sets to appropriate continual learning ones from \cite{harutyunyan2019multitask} to model the extreme case of a single model deployed on heterogeneous tasks sequentially through its life-cycle:


\subsection{Domain shift}
\label{sec:domain-shift}

We additionally include several domain-incremental learning problems splitting datasets by various demographics. First we consider \textbf{temporal} domain shift, where subsequent tasks refer to the same type of data and same problem statement, but recorded over different ranges of time (e.g. data split seasonally, or annually). This is representative of scenarios where due to data privacy constraints, samples cannot be retained after a certain time-period, even within one institution.

In such settings covariate shift may happen continuously, with overlap between tasks. We model such overlap explicitly in experiment \ref{...} (overlapping time periods for tasks), contrary to how many CL methods have previously been evaluated, where there are discrete boundaries between task distributions.

% We consider two types of temporal domain shift - 1) where there is a discrete boundary between tasks and 2) where there is overlap between subsequent tasks.

Note that due to anonymisation requirements, certain date elements have been removed or randomly shifted for all patients. eICU dates retain year granularity, but since they are only sampled over two years (2014-2015) is of low suitability for a continual learning experiment:

\begin{table}[ht]
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{lcccccc}
                  & \multicolumn{6}{c}{\textbf{Datetime element}}  \\
\textbf{Dataset}  & \multicolumn{1}{l}{\textbf{Time of day}} & \multicolumn{1}{l}{\textbf{Day of week}} & \multicolumn{1}{l}{\textbf{Day of month}} & \multicolumn{1}{l}{\textbf{Month}} & \multicolumn{1}{l}{\textbf{Seasonality}} & \multicolumn{1}{l}{\textbf{Year}} \\
\hyperlink{https://eicu-crd.mit.edu/eicutables/patient/}{eICU}    & \checkmark                                        &                                          &                                           &                                    &                                          & \checkmark                                 \\
\hyperlink{https://hirid.intensivecare.ai/}{HiRID}                & \checkmark                                        & \checkmark                                        &                                           &                                    & \checkmark                                        &                                   \\
\hyperlink{https://mimic.mit.edu/docs/iii/about/time/}{MIMIC-III} & \checkmark                                        & \checkmark                                        &                                           &                                    & \checkmark                                        &                                  
\end{tabular}
\end{adjustbox}
\end{table}

Secondly we consider \textbf{demographic} domain shift, where subsequent tasks refer to the same type of data but the population-level demographics differ between tasks (e.g. data split by hospital).

Examples of such tasks settings may be:

\begin{itemize}
    \item  different tasks refer to data collected from different hospitals, for data privacy reasons samples cannot be shared between institutions
    
    \item different tasks refer to recordings with different devices or models/versions of devices (e.g. ECG model 1 vs ECG model 2 etc)
    
    \item Different underlying factors (hospital A has antibiotic stewardship, hospital B does not etc)
    
\end{itemize}

% Evaluate methods on average performance over all random permutations of task ordering vs actual temporal ordering to show if any classes of methods perform better in the realistic scenario?

\subsubsection{Mitigating bias}

We further evaluate on artificial splits of the data by other demographics (gender, age, ethnicity) to evaluate the hypothetical scenario of an algorithm trained initially on a certain population but is found to have had little or no representation of a minority group, which is later specifically trained on data from these groups. \citet{thiagarajan2018understanding}

A more advanced version of this where the proportion of samples from the minority group in 

% IDEA #2: continual learning as mitigation for bias against minority classes???????
% Evaluate how model trained on x% majority class, (1-x%) minority class performs when subsequently trained on task 2 with 100% minority class (but smaller sample size for realism?)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Models have suffered criticism for bias with respect to minority groups. Such biases commonly stem from data imbalance. Training sets either non-representatively sample certain demographics, or sample from a population with inherent imbalance. 

%undersample due to training on datasets where minority groups are not sufficiently represented in order to .....)

Several architectural methods have been proposed to mitigate this, for example oversampling or inverse proportionate weighting of minority classes, but they ... 

% CITE facial paper that performs well only on white people and other examples. Cite fact sheet with breakdowns of accuracies on m/f age, ethnicity etc

Continual learning has a natural application in correcting such biases with the following framework:

1. identify pre-trained model which performs poorly on minority group
2. collect data from minority group
3. perform additional continual learning task on new data
4. repeat with as many groups as are identified as being under-represented

Here we evaluate the ability of continual learning methods to mitigate such bias once discovered. Given that in real-world scenarios one underlying hurdle to unbiased models is cost of collecting data from enough participants to sample a representative number of data points from minority groups, we construct subsequent tasks using at most a small proportion of the original task's dataset-size.

We provide an additional task empirically evaluating the effect on fairness of new tasks' dataset size.

% Age
% Ethnicity
% Gender

% Evaluate on examples from specific new task or total of group-members across all tasks?

\citet{churamani2021domain, kara2021towards} address this issue with respect to racial and gender bias in facial-recognition based systems. In their experiments, the domain incremental continual learning scenario is defined by splitting a single dataset into subsequent tasks by group identity of the subjects (split along race or gender). However this assumes access to all data as initially sampled, and does not provide a large increase in fairness (the measured metric) as compared to multi-task learning.

We explore an alternative setup here, where a population-representative dataset is used as task $T_1$ sampled from time period 1, and subsequent tasks refer to oversampled instances of only the minority group at time period 2, 3, etc. or from institution 2, 3 etc. I.e. general population from Hospital 1 comprises the data for task 1, for task 2 we sample only ethnic minority group $2$ from hospital 2, ..., for task n we sample only ethnic minority group $n$ from hospital $n$.


\begin{table}[ht]
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{cclr}
\multicolumn{2}{c}{Dataset}       &                              & \\
\textbf{MIMIC-III} & \textbf{eICU} & \textbf{Domain increment}   & \textbf{Number of domains} \\
                   & \checkmark    & Region (US)                 & 4    \\
                   & \checkmark    & Hospital                    & 155  \\
                   & \checkmark    & Unit                        & 8    \\
\checkmark         & \checkmark    & Sex                         & 2    \\
\checkmark         & \checkmark    & Age                         & 6-7  \\
\checkmark         & \checkmark    & Ethnicity (broad)           & 5    \\
\checkmark         &               & Ethnicity (narrow)          & ??   \\
\checkmark         &               & Time (season)               & 4    \\
\end{tabular}
\end{adjustbox}
\caption{Domain shifts exhibited in the MIMIC-III and eICU-CRD datasets. When multiple figures are given, these correspond to domains represented in subsets with different outcomes (i.e. mortality, Shock, ARF).}
\end{table}


\begin{table}[ht]
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{cc|l|lllllllllll}
\multicolumn{2}{c|}{Dataset}                        & \multicolumn{1}{c|}{\multirow{2}{*}{Domain increment}} & \multicolumn{11}{c}{Task}                                                                                                                                      \\
\textbf{MIMIC-III} & \textbf{eICU} & \multicolumn{1}{c|}{}                                  & \textbf{1}       & \textbf{2} & \textbf{3}    & \textbf{4}  & \textbf{5}    & \textbf{6}   & \textbf{7} & \textbf{8} & \textbf{9} & \textbf{...} & \textbf{28} \\ \hline
                   & \checkmark    & Hospital                                               & 73               & 110        & 122           & 142         & 167           & 176          & 183        & 188        & 197        & ...          & 458         \\
\checkmark         &               & Ethnicity                                              &                  &            &               &             &               &              &            &            &            &              &             \\
                   & \checkmark    & Unit                                                   & CCU              & CSICU      & CTICU         & Cardiac ICU & MICU          & Med-Surg ICU & Neuro ICU  & SICU       & -          & ...          & -           \\
\checkmark         & \checkmark    & Age                                                    & (0, 51{]}        & (51, 61{]} & (61, 69{]}    & (69, 78{]}  & (78, 89{]}    & 89 $\leq$    & -          & -          & -          & ...          & -           \\
\checkmark         & \checkmark    & Ethnicity (broad)                                      & African American & Asian      & Caucasian     & Hispanic    & Other/Unknown & -            & -          & -          & -          & ...          & -           \\
\checkmark         &               & Time (season)                                          & Spring           & Summer     & Autumn        & Winter      & -             & -            & -          & -          & -          & ...          & -           \\
                   & \checkmark    & Region (US)                                            & Northwest        & Midwest    & East          & South       & -             & -            & -          & -          & -          & ...          & -           \\
\checkmark         & \checkmark    & Sex                                                    & Female           & Male       & -             & -           & -             & -            & -          & -          & -          & ...          & -           \\
\end{tabular}
\end{adjustbox}
\caption{Here we show the domain shifts exhibited in the various Domain Incremental learning experiments.}
\end{table}

% Make table generation programmatic


\subsection{Label shift}

Clinical data may also undergo label shift when novel diseases present in the target population. We present the following class incremental problem:

\begin{itemize}
    \item Task 1: predict shock
    \item Task 2: predict ARF
    \item Task 3: predict mortality
\end{itemize}



We also propose a number of more representative TI and CI problems where tasks share a degree of inferred similarity (respiratory diseases?):

Class incremental:


- Task 1: no event vs shock
- Task 2: no event vs shock vs ARF
- Task 3: no event vs shock vs ARF vs mortality

% How is this different from CI?

We adapt the multi-task problem sets of \cite{harutyunyan2019multitask} to TI and CI continual learning problems on MIMIC-III as so (for full documentation, see Supplementary [XYZ]):

...

These are naturally converted to CL problems, by considering an ordering of tasks, and learning them sequentially as opposed to simultaneously.

(To avoid potentially biased performance due to a particular curriculum ordering, for unordered tasks we repeat the experiments over all orderings and average.)

As per the nature of Continual Learning, in a classification context each Task Incremental classification problem has an analogous Class Incremental problem, where the set of classes increases with each new task as opposed to replaced.

We generally find task incremental problems to be unrealistic scenarios for EHR where devices are deployed with a specific diagnostic - the field is yet immature to consider devices which are .....

%.................

One context in which Task/Class Incremental Learning may be realistically applicable to a clinical setting is in the emergence of novel diseases. Here, as data for a specific disease is encountered, the initial task is identifying patients with/without the disease. As novel diseases emerge in the population, subsequent tasks become non-disease vs disease$_1$ vs disease$_2$ etc.

Such a 

%-------------------

To exemplify such scenarios we provide the following training problems also derived from MIMIC-III:

\begin{table}[ht]
\begin{tabular}{l|lll}
                                                                         & \textbf{Task 1}     & \textbf{Task 2}                    & \textbf{Task 3}                           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Respiratory \\ diseases\end{tabular}} & None vs influenza   & None vs influenza vs ... H1N1      & None vs influenza vs H1N1 vs ...          \\
\textbf{\begin{tabular}[c]{@{}l@{}}AMR \\ varieties\end{tabular}}        & None vs X-resistant & None vs X-resistant vs Y-resistant & None vs X-resistant vs Y-resistant vs ...
\end{tabular}
\caption{Here we exemplify some Class Incremental problems in a clinical diagnostics scenario. A model is trained to identify a certain disease when apparent in the population. As similar diseases emerge in time, it is not only important to identify these but to determine which condition the patient has.}
\label{tab:class-inc}
\end{table}


\begin{figure}[t]
	\centering
	\includegraphics[width=8cm]{figs/fig5}
	\caption{Here we see 3 sequential tasks: dark blue, light blue, grey. Data for each task is split temporally into training (first 70\%) and test (final 30\%, dashed border).}
	\label{fig:figs/split-by-time}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\paragraph{Domain Adaptation} Continual learning has similar goals to the field of \textit{Domain Adaptation} (DA). Both fields are concerned with methods to adapting a model trained on a source domain to a target domain. The major differences are:

\begin{table}[b]
\centering
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular} {l|ll}
 & \textbf{Domain Adaptation}   & \textbf{Continual Learning}     \\ \hline
$n$ domains                        & 2 (source, target)  & $n \geq 2$  \\
Access to prior domains' data      & \checkmark & \xmark \footnote{Rehearsal methods violate this assumption.}   \\
Avoids catastrophic forgetting     & \xmark     & \checkmark
\end{tabular}
\end{adjustbox}
\caption{Comparison of Domain Adaptation with Continual Learning. 1. Rehearsal methods violate this assumption.}
\label{tab:domain-v-cl}
\end{table}

Note in this sense Domain Adaptation is analogous to Domain incremental continual learning, as transfer learning is analogous to continual learning generally.

==> table_boilerplate.tex <==
\begin{table*}[ht]
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{clllllllllllllll}
                       &                       & \multicolumn{14}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Temporal Domain Increment\end{tabular}}}                                                        \\
\multicolumn{2}{c|}{\multirow{2}{*}{CL Method}}                  & \multicolumn{4}{c}{Time (season)}             & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Region (US)}           & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Hospital unit} \\
\multicolumn{2}{c|}{}           & MLP & CNN & LSTM & \multicolumn{1}{l|}{Transformer} &                      & MLP & CNN & LSTM & \multicolumn{1}{l|}{Transformer} &                      & MLP    & CNN    & LSTM  & Transformer   \\ \hline
\multirow{2}{*}{Baseline}       & \multicolumn{1}{l|}{Naive}     & ... & ... & ... & \multicolumn{1}{l|}{...}  &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{Joint}     &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{}          &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multirow{4}{*}{Regularization} & \multicolumn{1}{l|}{EWC}       &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{Online EWC}&     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{SI}        &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{LwF}       &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multicolumn{1}{l}{}            & \multicolumn{1}{l|}{}          &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multirow{3}{*}{Rehearsal}      & \multicolumn{1}{l|}{Replay}    &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{GEM}       &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{A-GEM}     &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multicolumn{1}{l}{}            & \multicolumn{1}{l|}{}          &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        
\end{tabular}
\end{adjustbox}

\bigskip

\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{clllllllllllllll}
                       &                       & \multicolumn{14}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Demographic Domain Increment\end{tabular}}}                                                        \\
\multicolumn{2}{c|}{\multirow{2}{*}{CL Method}}                  & \multicolumn{4}{c}{Age}             & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Ethnicity (broad)}           & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Ethnicity (narrow)} \\
\multicolumn{2}{c|}{}           & MLP & CNN & LSTM & \multicolumn{1}{l|}{Transformer} &                      & MLP & CNN & LSTM & \multicolumn{1}{l|}{Transformer} &                      & MLP    & CNN    & LSTM  & Transformer   \\ \hline
\multirow{2}{*}{Baseline}       & \multicolumn{1}{l|}{Naive}     & ... & ... & ... & \multicolumn{1}{l|}{...}  &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{Joint}     &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{}          &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multirow{4}{*}{Regularization} & \multicolumn{1}{l|}{EWC}       &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{Online EWC}&     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{SI}        &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{LwF}       &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multicolumn{1}{l}{}            & \multicolumn{1}{l|}{}          &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multirow{3}{*}{Rehearsal}      & \multicolumn{1}{l|}{Replay}    &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{GEM}       &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{A-GEM}     &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multicolumn{1}{l}{}            & \multicolumn{1}{l|}{}          &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        
\end{tabular}
\end{adjustbox}

\bigskip

\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{clllllllllllllll}
                       &                       & \multicolumn{14}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Geographic Domain Increment\end{tabular}}}                                                        \\
\multicolumn{2}{c|}{\multirow{2}{*}{CL Method}}                  & \multicolumn{4}{c}{Hospital $(n=20)$}             & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Hospital $(n=50)$}           & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Hospital $(n=100)$} \\
\multicolumn{2}{c|}{}           & MLP & CNN & LSTM & \multicolumn{1}{l|}{Transformer} &                      & MLP & CNN & LSTM & \multicolumn{1}{l|}{Transformer} &                      & MLP    & CNN    & LSTM  & Transformer   \\ \hline
\multirow{2}{*}{Baseline}       & \multicolumn{1}{l|}{Naive}     & ... & ... & ... & \multicolumn{1}{l|}{...}  &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{Joint}     &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{}          &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multirow{4}{*}{Regularization} & \multicolumn{1}{l|}{EWC}       &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{Online EWC}&     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{SI}        &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{LwF}       &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multicolumn{1}{l}{}            & \multicolumn{1}{l|}{}          &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multirow{3}{*}{Rehearsal}      & \multicolumn{1}{l|}{Replay}    &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{GEM}       &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
                                & \multicolumn{1}{l|}{A-GEM}     &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        \\
\multicolumn{1}{l}{}            & \multicolumn{1}{l|}{}          &     &     &     & \multicolumn{1}{l|}{}     &                      &     &     &     & \multicolumn{1}{l|}{}     &                      &        &        &       &        
\end{tabular}
\end{adjustbox}
\caption{Final average performance for 48hr mortality prediction across temporal domain shift (top) and geographic domain shift (bottom). Progressive neural networks (PNN) as originally defined could only be applied to the simple feedforward network (MLP).}
\label{tab:results}
\end{table*}
